Virtual Private Mobile Network with Multiple Gateways for B5G Location Privacy

In a beyond-5G (B5G) scenario, we consider a virtual private mobile network (VPMN), i.e., a set of user equipments (UEs) directly communicating in a device-to-device (D2D) fashion, and connected to the cellular network by multiple gateways. The purpose of the VPMN is to hide the position of the VPMN UEs to the mobile network operator (MNO). We investigate the design and performance of packet routing inside the VPMN. First, we note that the routing that maximizes the rate between the VPMN and the cellular network leads to an unbalanced use of the gateways by each UE. In turn, this reveals information on the location of the VPMN UEs. Therefore, we derive a routing algorithm that maximizes the VPMN rate, while imposing for each UE the same data rate at each gateway, thus hiding the location of the UE. We compare the performance of the resulting solution, assessing the location privacy achieved by the VPMN, and considering both the case of single hop and multihop in the transmissions from the UEs to the gateways.

==> draft (copy)/otros/BORRAR.tex <==


\newpage

\begin{equation}
\begin{aligned}
\max_{f\in\mathbb{R}} \quad & \sum_{v:(v,s_i)} f_{v,s_i}\\
\textrm{s.t.} \quad & f_{i,j}\leq c_{i,j} \quad \forall (i,j) \in U\\
  & \sum_{i} f_{i,k}\leq\sum_{j} f_{k,j} \quad \forall k \neq s_m\quad m=1,2,...,M  \\
  & f_{i,j} \geq 0 \quad \forall (i,j) \in U
\end{aligned}
\end{equation}

==> draft (copy)/otros/channelmodel_con_ij.tex <==
We consider a model with a single cell of size $MxM$ meters where we let $N$ denote the number of nodes which are randomly distributed around the map in a in-coverage urban scenario. This map constitutes a VPMN where the users communicate with each other without routing information to the gNB. We consider that all couples of nodes are in line-of-sight (LOS). For simplicity, we consider a two-dimensional scenario where the vertical dimension is ignored. \par
In the simplest model \cite{1111111}, all nodes are considered to work as generic relays. This means that any of the UEs in the VPMN can act as a relay of the gNB to obtain coverage. The only requirement for the communication of the nodes is that the euclidean distance $d_{i,j}$ between them is lower than a threshold, that is $d_{i,j} < d_{min}$. Following this, the connected component to a specific UE is obtained as the group of UEs that fulfill that requirement, creating the VPMN. In the mentioned paper, the uncertainty of the position of a UE is studied represented as the maximum distance between the selected UE and the farthest VPMN UE.\par

\section{Our system} %This must change but I want to divide it somehow
Starting from the model mentioned above, now we want to make the system more complex, adding to the distance condition the effects of shadowing and path loss in a urban scenario. As in \cite{4024752}, we will assume the spatially correlated shadowing, specifically the log-normal shadowing $Y$ and the propagation loss with path loss exponent $\alpha$. The value used to check the connection between nodes will be the carrier-to-noise ratio (CNR) $\Gamma(d)$, which considers both the shadowing and the path loss. We also use a normalization factor $r_0$. 

\begin{equation} \label{eq:1}
    \Gamma_{i,j}(d)=Y_{i,j}*\left(\frac{d_{i,j}}{r_0}\right)^{-\alpha}
\end{equation}
where $\Gamma_{i,j}$, $Y_{i,j}$ and $d_{i,j}$ are matrices of size NxN-1. This design decision is taken so that the distance between self-nodes is not considered, so the diagonal of the distance matrix is removed, thus making it easier to work with it later. \par
In order to obtain the spatially correlated shadowing, we need the correlation between the couples of nodes of the network, obtained as follows:

\begin{equation}
    R_{i,j}=exp\left(-\frac{d_{i,j}}{d_{cor}}*ln2\right)
\end{equation}

where $d_{cor}$ is the decorrelation distance, dependent on the environment: 20 meters for an urban environment. In this case, the size of $R_{i,j}$ is NxN, as we require that it is symmetric, square and positive definite to apply the following steps. \par
After the correlation coefficients have been obtained, we want to obtain a matrix $Y$ of Gaussian distributed random variables which are correlated with correlation coefficients given by the matrix $R$, which will be the shadowing values for the N receivers. We will achieve this by creating a matrix of standard Gaussian random variables $x\sim \mathcal{N}(0,1)$. This matrix will be multiplied by a matrix $L$ that makes the resulting random variables in the matrix be correlated. This is achieved by substituting: 
\begin{equation} \label{eq:2}
    \textbf{Y}=\textbf{Lx}
\end{equation}
\begin{gather*}
    E[Y^HY]=R \xrightarrow{} E[L^Hx^HLx]=R \xrightarrow{} L*E[xx^H]*L^H=R
\end{gather*}
\begin{equation}
    R=LL^H
\end{equation}

Once $R$ is obtained, $L$ can be resolved by the Cholesky factorization. The only requirement is that the matrix $L$ is positive definite, which is guaranteed in this specific case. When L is computed, $Y$ is acquired in (\ref{eq:2}) and thus (\ref{eq:1}) can be calculated. \par
After all, each couple of nodes will be evaluated through a threshold both for the distance between the nodes, $d_{min}$ and the value of the CNR, $\Gamma_{th}$ to determine whether they can be connected or not. 

==> draft (copy)/otros/maxflow.tex <==
\chapter{Maximum Flow}
\section{Multiple Sources Single Sink}
Let a graph $G=(V,U)$ represent a network where $V$ are the nodes, which we will call sources, and $U$ the links between nodes. Let $N$ be the number of sources, denoted as $v_n$ with $n=1,2,...,N$. The cell contains a single sink $s$ where all the data is directed to. Each link has a capacity $c_{i,j}$ between sources $v_i$ and $v_j$. Between each link from source $v_i$ to $v_j$ there is a flow $f_{i,j}$.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\textwidth]{images/dibujo.png}
    \caption{Maximum flow problem with multiple sources and single sink.}
    \label{fig:msss}
\end{figure}

\autoref{fig:msss} shows a basic representation of the network, including some sources and the single sink. Now we also want to consider that each source generates data (flow), which means that the source has a capacity $c_n$, with $n=1,2,...,N$. 

The optimization problem to obtain the maximum rate is expressed as:

\begin{equation}
\begin{aligned}
\max_{f\in\mathbb{R}} \quad & \sum_{v:(v,s)} f_{v,s}\\
\textrm{s.t.} \quad & f_{i,j}\leq c_{i,j} \quad \forall (i,j) \in U\\
  & \sum_{i} f_{i,k}\leq\sum_{j} f_{k,j} \quad \forall k \neq s  \\
  & f_{i,j} \geq 0 \quad \forall (i,j) \in U
\end{aligned}
\end{equation}

The objective is to maximize the flow going to the sink $s$. We have three conditions: the first one is the capacity condition, where the flow through a link cannot exceed the capacity of the link. The second one is the flow conservation but applied to our problem, where we let source $k$ generate a flow of $(f_{i,k}-f_{k,j})$ bit/s. The third one represents that we cannot have a negative flow.

\section{Multiple Sources Multiple Sinks}
Now we have the same problem as in the previous section, but in this case with multiple sinks. We let $M$ denote the number of sinks, named $s_m$ with $m=1,2,...,M$. Each link has still a capacity $c_{i,j}$ and the flow between each link is $f_{i,j}$. In this case, for each source we will fix the sink that it is connected to. This assignment will not follow the 'closest-sink' criterion, as it would reduce the uncertainty in the position of the sources and thus the privacy of the users of the VPMN.  

\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\textwidth]{images/dibujomsms.png}
    \caption{Maximum flow problem with multiple sources and sinks.}
    \label{fig:msms}
\end{figure}

\autoref{fig:msms} represents a simple network containing 3 sources and 2 sinks. As in the previous case, each source will generate flow with a capacity $c_n$, with $n=1,2,...,N$. One way of solving these types of networks is reducing the problem of multiple sources and multiple sinks to an ordinary maximum flow problem with a single source and single sink.

The optimization problem is now written as:



==> otros/BORRAR.tex <==


\newpage

\begin{equation}
\begin{aligned}
\max_{f\in\mathbb{R}} \quad & \sum_{v:(v,s_i)} f_{v,s_i}\\
\textrm{s.t.} \quad & f_{i,j}\leq c_{i,j} \quad \forall (i,j) \in U\\
  & \sum_{i} f_{i,k}\leq\sum_{j} f_{k,j} \quad \forall k \neq s_m\quad m=1,2,...,M  \\
  & f_{i,j} \geq 0 \quad \forall (i,j) \in U
\end{aligned}
\end{equation}

==> otros/channelmodel_con_ij.tex <==
We consider a model with a single cell of size $MxM$ meters where we let $N$ denote the number of nodes which are randomly distributed around the map in a in-coverage urban scenario. This map constitutes a VPMN where the users communicate with each other without routing information to the gNB. We consider that all couples of nodes are in line-of-sight (LOS). For simplicity, we consider a two-dimensional scenario where the vertical dimension is ignored. \par
In the simplest model \cite{1111111}, all nodes are considered to work as generic relays. This means that any of the UEs in the VPMN can act as a relay of the gNB to obtain coverage. The only requirement for the communication of the nodes is that the euclidean distance $d_{i,j}$ between them is lower than a threshold, that is $d_{i,j} < d_{min}$. Following this, the connected component to a specific UE is obtained as the group of UEs that fulfill that requirement, creating the VPMN. In the mentioned paper, the uncertainty of the position of a UE is studied represented as the maximum distance between the selected UE and the farthest VPMN UE.\par

\section{Our system} %This must change but I want to divide it somehow
Starting from the model mentioned above, now we want to make the system more complex, adding to the distance condition the effects of shadowing and path loss in a urban scenario. As in \cite{4024752}, we will assume the spatially correlated shadowing, specifically the log-normal shadowing $Y$ and the propagation loss with path loss exponent $\alpha$. The value used to check the connection between nodes will be the carrier-to-noise ratio (CNR) $\Gamma(d)$, which considers both the shadowing and the path loss. We also use a normalization factor $r_0$. 

\begin{equation} \label{eq:1}
    \Gamma_{i,j}(d)=Y_{i,j}*\left(\frac{d_{i,j}}{r_0}\right)^{-\alpha}
\end{equation}
where $\Gamma_{i,j}$, $Y_{i,j}$ and $d_{i,j}$ are matrices of size NxN-1. This design decision is taken so that the distance between self-nodes is not considered, so the diagonal of the distance matrix is removed, thus making it easier to work with it later. \par
In order to obtain the spatially correlated shadowing, we need the correlation between the couples of nodes of the network, obtained as follows:

\begin{equation}
    R_{i,j}=exp\left(-\frac{d_{i,j}}{d_{cor}}*ln2\right)
\end{equation}

where $d_{cor}$ is the decorrelation distance, dependent on the environment: 20 meters for an urban environment. In this case, the size of $R_{i,j}$ is NxN, as we require that it is symmetric, square and positive definite to apply the following steps. \par
After the correlation coefficients have been obtained, we want to obtain a matrix $Y$ of Gaussian distributed random variables which are correlated with correlation coefficients given by the matrix $R$, which will be the shadowing values for the N receivers. We will achieve this by creating a matrix of standard Gaussian random variables $x\sim \mathcal{N}(0,1)$. This matrix will be multiplied by a matrix $L$ that makes the resulting random variables in the matrix be correlated. This is achieved by substituting: 
\begin{equation} \label{eq:2}
    \textbf{Y}=\textbf{Lx}
\end{equation}
\begin{gather*}
    E[Y^HY]=R \xrightarrow{} E[L^Hx^HLx]=R \xrightarrow{} L*E[xx^H]*L^H=R
\end{gather*}
\begin{equation}
    R=LL^H
\end{equation}

Once $R$ is obtained, $L$ can be resolved by the Cholesky factorization. The only requirement is that the matrix $L$ is positive definite, which is guaranteed in this specific case. When L is computed, $Y$ is acquired in (\ref{eq:2}) and thus (\ref{eq:1}) can be calculated. \par
After all, each couple of nodes will be evaluated through a threshold both for the distance between the nodes, $d_{min}$ and the value of the CNR, $\Gamma_{th}$ to determine whether they can be connected or not. 

==> otros/maxflow.tex <==
\chapter{Maximum Flow}
\section{Multiple Sources Single Sink}
Let a graph $G=(V,U)$ represent a network where $V$ are the nodes, which we will call sources, and $U$ the links between nodes. Let $N$ be the number of sources, denoted as $v_n$ with $n=1,2,...,N$. The cell contains a single sink $s$ where all the data is directed to. Each link has a capacity $c_{i,j}$ between sources $v_i$ and $v_j$. Between each link from source $v_i$ to $v_j$ there is a flow $f_{i,j}$.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\textwidth]{images/dibujo.png}
    \caption{Maximum flow problem with multiple sources and single sink.}
    \label{fig:msss}
\end{figure}

\autoref{fig:msss} shows a basic representation of the network, including some sources and the single sink. Now we also want to consider that each source generates data (flow), which means that the source has a capacity $c_n$, with $n=1,2,...,N$. 

The optimization problem to obtain the maximum rate is expressed as:

\begin{equation}
\begin{aligned}
\max_{f\in\mathbb{R}} \quad & \sum_{v:(v,s)} f_{v,s}\\
\textrm{s.t.} \quad & f_{i,j}\leq c_{i,j} \quad \forall (i,j) \in U\\
  & \sum_{i} f_{i,k}\leq\sum_{j} f_{k,j} \quad \forall k \neq s  \\
  & f_{i,j} \geq 0 \quad \forall (i,j) \in U
\end{aligned}
\end{equation}

The objective is to maximize the flow going to the sink $s$. We have three conditions: the first one is the capacity condition, where the flow through a link cannot exceed the capacity of the link. The second one is the flow conservation but applied to our problem, where we let source $k$ generate a flow of $(f_{i,k}-f_{k,j})$ bit/s. The third one represents that we cannot have a negative flow.

\section{Multiple Sources Multiple Sinks}
Now we have the same problem as in the previous section, but in this case with multiple sinks. We let $M$ denote the number of sinks, named $s_m$ with $m=1,2,...,M$. Each link has still a capacity $c_{i,j}$ and the flow between each link is $f_{i,j}$. In this case, for each source we will fix the sink that it is connected to. This assignment will not follow the 'closest-sink' criterion, as it would reduce the uncertainty in the position of the sources and thus the privacy of the users of the VPMN.  

\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\textwidth]{images/dibujomsms.png}
    \caption{Maximum flow problem with multiple sources and sinks.}
    \label{fig:msms}
\end{figure}

\autoref{fig:msms} represents a simple network containing 3 sources and 2 sinks. As in the previous case, each source will generate flow with a capacity $c_n$, with $n=1,2,...,N$. One way of solving these types of networks is reducing the problem of multiple sources and multiple sinks to an ordinary maximum flow problem with a single source and single sink.

The optimization problem is now written as:


